Towards Robust Unsupervised Disentanglement of Sequential Data -- A Case Study Using Music Audio

Disentangled sequential autoencoders (DSAEs) represent a class of probabilistic graphical models that describes an observed sequence with dynamic latent variables and a static latent variable. The former encode information at a frame rate identical to the observation, while the latter globally governs the entire sequence. This introduces an inductive bias and facilitates unsupervised disentanglement of the underlying local and global factors. In this paper, we show that the vanilla DSAE suffers from being sensitive to the choice of model architecture and capacity of the dynamic latent variables, and is prone to collapse the static latent variable. As a countermeasure, we propose TS-DSAE, a two-stage training framework that first learns sequence-level prior distributions, which are subsequently employed to regularise the model and facilitate auxiliary objectives to promote disentanglement. The proposed framework is fully unsupervised and robust against the global factor collapse problem across a wide range of model configurations. It also avoids typical solutions such as adversarial training which usually involves laborious parameter tuning, and domain-specific data augmentation. We conduct quantitative and qualitative evaluations to demonstrate its robustness in terms of disentanglement on both artificial and real-world music audio datasets.

==> sections/conclusion.tex <==
 

==> sections/draft.tex <==
%Having been concerned with learning a single global factor, 
We now consider both the fourth and fifth octaves when synthesising the dMelodies dataset, introducing octave number as the other global factor of variation in addition to instrument identity.
We train the decoder-enriched TS-DSAE described in \secref{sec:rich_decoder}, and show the results in \figref{fig:multiple}.
In particular, we replace $\bv{v}$ inferred from the source at the lower left, with that derived from one of the three targets displayed in the top row, and generate novel samples shown from the second to last columns of the bottom row.

We use $\{i, o, m\}$ to denote the instrument, octave, and melody of each sample, respectively.
%, where $i\in\{i_1, i_2\}$, $o\in\{o_1, o_2\}$, and $m\in\{m_1, m_2, m_3, m_4\}$.
For example, the source $\{i_1, o_1, m_1\}$ and the first target $\{i_2, o_1, m_2\}$ share the same octave but differ in the instrument, characterised by the spectral distribution along the frequency axis.
As a result of replacing $\bv{v}$, the target instrument $i_2$ is manifested in the outcome $\{i_{1\rightarrow2}, o_1, m_1\}$, while the octave remains unchanged.
Similarly, the second target $\{i_1, o_2, m_3\}$ differs from the source with the octave, characterised by the level of pitch contour; therefore, swapping $\bv{v}$ only transforms the octave for the output $\{i_1, o_{1\rightarrow2}, m_1\}$.
Finally, the sample $\{i_{1\rightarrow2}, o_{1\rightarrow2}, m_1\}$ results from using the target $\{i_2, o_2, m_4\}$ that does not share any of the attributes with the source, where both the instrument and octave are converted.
Importantly, the source melody $m_1$ remains intact in the three transformed samples, suggesting the global-local disentanglement.


==> tables/dsaF_dmel_global.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline

\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA(Full)}                                                                                    \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 75.06    & 23.16       & 24.79      & 54.66    & 39.49       & 36.97      & 73.84    & 25.56       & 27.27       \\
Prg-F                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 0.00        & 0.00        \\
Prg                  & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00      \\
Prg-C                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00      \\
\hline
\end{tabular}
\caption{DSA(Full), dMel, global}
\end{table*}

==> tables/dsaF_dmel_local.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA(Full)}                                                                                    \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 93.51    & 93.49       & 93.18      & 93.54    & 93.59       & 93.28      & 93.32    & 93.43       & 93.07       \\
Prg-F                & 93.78    & 89.02       & 88.23      & 93.60    & 89.97       & 89.18      & 93.60    & 92.99       & 92.61       \\
Prg                  & 93.70    & 88.52       & 87.69      & 93.81    & 89.60       & 89.25      & 93.79    & 90.65       & 90.35       \\
Prg-C                & 93.60    & 87.56       & 86.44      & 93.68    & 88.91       & 88.21      & 93.54    & 90.42       & 89.99       \\
\hline
\end{tabular}
\caption{DSA(Full), dMel, local}
\end{table*}

==> tables/dsaF_urmp_global.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline

\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA(Full)}                                                                                    \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 100.00   & 97.52       & 96.42      & 76.97    & 15.83       & 26.76      & 93.29    & 4.96        & 10.81       \\
Prg-F                & 99.49    & 90.70       & 90.86      & 100.00   & 80.08       & 92.66      & 99.49    & 20.17       & 35.74       \\
Prg                  & 99.49    & 83.39       & 90.94      & 100.00   & 18.06       & 18.93      & 99.49    & 39.29       & 45.67       \\
Prg-C                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00      \\
\hline
\end{tabular}
\caption{DSA(Full), URMP, global}
\end{table*}


==> tables/dsaF_urmp_local.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA(Full)}                                                                                    \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 85.20    & 83.96       & 73.65      & 85.08    & 84.67       & 86.60      & 85.00    & 84.90       & 86.49       \\
Prg-F                & 85.52    & 84.80       & 74.24      & 85.09    & 82.59       & 75.12      & 84.90    & 80.53       & 75.05       \\
Prg                  & 85.35    & 84.17       & 75.20      & 85.16    & 82.93       & 80.81      & 85.17    & 82.44       & 75.87       \\
Prg-C                & 85.24    & 82.10       & 75.02      & 84.65    & 83.09       & 74.78      & 84.90    & 82.65       & 76.21       \\
\hline
\end{tabular}
\caption{DSA(Full), URMP, local}
\end{table*}


==> tables/dsa_dmel_global.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA}                                                                                          \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 53.73    & 46.05       & 41.96      & 67.73    & 30.36       & 31.96      & 52.25    & 47.22       & 50.70       \\
Prg-F                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 0.00        & 0.00        \\
Prg                  & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 88.66       & 92.16       \\
Prg-C                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00      \\ 
\hline
\end{tabular}
\caption{DSA, dMel, global}
\end{table*}


==> tables/dsa_dmel_local.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA}                                                                                          \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 93.49    & 93.49       & 93.12      & 93.68    & 93.65       & 93.31      & 93.51    & 93.53       & 93.21       \\
Prg-F                & 93.81    & 91.17       & 90.72      & 93.81    & 91.76       & 91.34      & 93.78    & 93.56       & 93.28       \\
Prg                  & 93.52    & 90.25       & 89.69      & 93.49    & 91.10       & 90.80      & 93.70    & 91.35       & 91.32       \\
Prg-C                & 93.10    & 89.03       & 88.35      & 93.39    & 90.13       & 89.42      & 93.51    & 90.94       & 90.51       \\ 
\hline
\end{tabular}
\caption{DSA, dMel, local}
\end{table*}



==> tables/dsa_urmp_global.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA}                                                                                          \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 94.44    & 4.22        & 5.79       & 91.52    & 6.01        & 12.04      & 82.24    & 11.22       & 22.61       \\
Prg-F                & 100.00   & 70.98       & 70.93      & 100.00   & 60.36       & 60.95      & 100.00   & 17.68       & 25.74       \\
Prg                  & 100.00   & 79.61       & 81.42      & 100.00   & 87.81       & 86.01      & 100.00   & 28.35       & 41.80       \\
Prg-C                & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00     & 100.00   & 100.00      & 100.00      \\ 
\hline
\end{tabular}
\caption{DSA, URMP, global}
\end{table*}



==> tables/dsa_urmp_local.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|lll|lll|lll} 
\hline
\multicolumn{1}{l}{} & \multicolumn{9}{l}{DSA}                                                                                          \\ 
\cline{2-10}
\multicolumn{1}{l}{} & \multicolumn{3}{l|}{8}              & \multicolumn{3}{l|}{16}             & \multicolumn{3}{l}{32}               \\ 
\cline{2-10}
\multicolumn{1}{l}{} & original & swap global & swap local & original & swap global & swap local & original & swap global & swap local  \\ 
\hline
Base                 & 84.80    & 84.70       & 85.87      & 85.40    & 85.35       & 86.02      & 84.55    & 84.52       & 85.94       \\
Prg-F                & 85.28    & 85.40       & 78.15      & 85.40    & 83.92       & 78.78      & 84.89    & 83.29       & 80.54       \\
Prg                  & 85.51    & 86.36       & 77.92      & 85.51    & 83.58       & 78.33      & 84.87    & 83.31       & 77.85       \\
Prg-C                & 82.82    & 70.07       & 62.75      & 84.72    & 82.75       & 73.05      & 85.35    & 84.60       & 77.72       \\ 
\hline

\end{tabular}
\caption{DSA, URMP, local}
\end{table*}



==> tables/fad_dmel.tex <==
\begin{table}
\small
\centering
\begin{tabular}{l|lll|lll} 
\hline
      & \multicolumn{3}{l|}{DSA} & \multicolumn{3}{l}{DSA(Full)}  \\ 
\cline{2-7}
      & 8    & 16   & 32         & 8    & 16   & 32               \\ 
\hline
Base  & 1.25 & 0.94 & 0.91       & 1.22 & 0.95 & 0.79             \\
Prg-F & 0.96 & 0.97 & 0.79       & 1.10 & 0.88 & 0.74             \\
Prg   & 1.24 & 0.97 & 0.79       & 1.25 & 0.85 & 0.86             \\
Prg-C & 2.00 & 1.49 & 1.34       & 1.34 & 1.13 & 0.97             \\
\hline
\end{tabular}
\caption{dMel, FAD}
\end{table}

==> tables/fad_urmp.tex <==
\begin{table}
\small
\centering
\begin{tabular}{l|lll|lll} 
\hline
      & \multicolumn{3}{l|}{DSA} & \multicolumn{3}{l}{DSA(Full)}  \\ 
\cline{2-7}
      & 8    & 16   & 32         & 8    & 16   & 32               \\ 
\hline
Base  & 5.45 & 4.54 & 3.92       & 7.12 & 5.77 & 4.60             \\
Prg-F & 5.18 & 4.22 & 3.34       & 6.84 & 5.45 & 4.73             \\
Prg   & 5.31 & 4.18 & 3.38       & 6.34 & 5.12 & 4.48             \\
Prg-C & 7.93 & 7.15 & 5.80       & 9.30 & 7.45 & 5.99             \\
\hline
\end{tabular}
\caption{URMP, FAD}
\end{table}
